TileLang: A Composable Tiled Programming Model for AI Systems

Modern AI workloads rely heavily on optimized computing kernels for both training and inference. These AI kernels follow well-defined data-flow patterns, such as moving tiles between DRAM and SRAM and performing a sequence of computations on those tiles. However, writing high-performance kernels remains complex despite the clarity of these patterns. Achieving peak performance requires careful, hardware-centric optimizations to fully leverage modern accelerators. While domain-specific compilers attempt to reduce the burden of writing high-performance kernels, they often struggle with usability and expressiveness gaps. In this paper, we present TileLang, a generalized tiled programming model for more efficient AI Kernel programming. TileLang decouples scheduling space (thread binding, layout, tensorize and pipeline) from dataflow, and encapsulated them as a set of customization annotations and primitives. This approach allows users to focus on the kernel's data-flow itself, while leaving most other optimizations to compilers. We conduct comprehensive experiments on commonly-used devices, across numerous experiments, our evaluation shows that TileLang can achieve state-of-the-art performance in key kernels, demonstrating that its unified block-and-thread paradigm and transparent scheduling capabilities deliver both the power and flexibility demanded by modern AI system development.

==> JIT.tex <==
\section{\oursys{} JIT Compiler}

\oursys{} JIT Compiler combines hardware-agnostic and hardware-aware optimization techniques to deliver high-performance code generation across diverse platforms. By automating tasks like software pipeline inference, loop tail split, and dead code elimination, \oursys{} ensures efficient and portable execution. Additionally, architecture-specific features such as warp specialization and memory optimizations allow \oursys{} to fully exploit modern hardware capabilities, striking a balance between generality and peak performance.

\subsection{Hardware Agnostic Optimizations}

\subsubsection{Software Pipeline Inference and Implementation}
\label{subsection:software_pipline_jit}



\subsubsection{Loop Tail Split for Dynamic Shapes}

% \LEI{In \oursys{}, the Loop Tail Split feature has been implemented to optimize tensor operations involving dynamic shapes by generating code with vectorized memory access. For example, when users specify matrices with dimensions that are determined at runtime, this feature assesses whether the dynamic dimensions satisfy the criteria for vectorization. If they do, the vectorized portion of the load process is extracted and encapsulated within a conditional statement, effectively separating it from the serialized portion of the code. This separation ensures that when the conditions for vectorization are met, the optimized vectorized code path is executed, thereby enhancing performance.}

\Zhengju{In \oursys{}, the Loop Tail Split optimization has been implemented to generate code with vectorized memory access for tensors with dynamic shapes. For instance, if the matrices to be loaded have their dimensions determined by users, this feature checks when these dynamic dimensions meet the requirement of vectorization. The vectorized part of the load process will then be extracted with a conditional statement to be separated from the serialized part, ensuring better performance through vectorization.}

\begin{figure}[t]
    \centering
    \vspace{-1mm}
    \includegraphics[width=\linewidth]{figures/looptailsplit-cropped.pdf}
    \vspace{-5mm}
    \caption{Potential Vectorized Memory Access Extracted from Loop Tail Split. Assume Vectorization Requires Memory Aligned to 8 Bytes.}
    \label{fig:looptailsplit}
\end{figure}

\subsubsection{Dead Code Elimination for Dynamic Arguments}
\LEI{Dead Code Elimination\cite{Cytron1991} (DCE) is a fundamental optimization technique employed by traditional compilers to enhance program efficiency. In conventional compilation workflows, DCE identifies and removes code segments that do not affect the program's observable behavior, including unused variables, unreachable code blocks, and redundant computations, thereby reducing code size and improving execution performance. In \oursys{}, DCE is not only implemented for dead statements, but also specifically designed to optimize templates with dynamic arguments in kernel functions. For example, in a general dequantization computation where a particular parameter is not utilized, \oursys{}'s DCE removes the unused parameter from the execution path and eliminates any associated conditional code that would have been executed based on that parameter. This comprehensive approach allows users to design programming templates with arbitrary parameters, maintains the generality of dynamic templates.}

% \Zhengju{The Dead Code Elimination (DCE) feature has been implemented to optimize templates with dynamic arguments in kernel functions. For instance, in a general dequantization computation, if a specific parameter is not utilized, this DCE feature eliminates the unused parameter from the execution path. This optimization reduces overhead and allows users to write flexible programming templates with arbitrary parameters, without worrying about performance penalties from unused arguments. By streamlining the computation process, this approach ensures better efficiency while maintaining the generality of dynamic templates.}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/DCE-cropped.pdf}
    \vspace{-2mm}
    \caption{Flexible Programming Template with Arbitrary Parameter via DCE.}
    \label{fig:DCE}
\end{figure}

\subsection{Hardware Aware Optimizations}

\subsubsection{Multi-Stage Layout Inference}


==> RelatedWork.tex <==
\section{RELATED WORK}


\para{Deep learning compilers and frameworks.}
Most existing deep learning compilers, such as ~\cite{chen2018tvm, zheng2020ansor,ma2020rammer, zhu2022roller,welder,zhang2023cocktailer,paszke2019pytorch,zheng2023pit,ansel2024pytorch}, focus on operator or model computation optimizations for mainstream data types, e.g., FP16 or FP32, with little emphasis on low-precision data types.
\rev{However, many optimizations are complementary with low-precision computing, for example, Roller~\cite{zhu2022roller} is leveraged to infer efficient \ttile{} configurations, and Welder~\cite{welder} is leveraged for end-to-end graph optimization in \oursys{}.}
\rev{SparTA~\cite{zheng2022sparta} treats model pruning and quantization as model sparsity to holistically optimize sparse model inference and training, and \oursys{} can provide efficient low-precision kernels to further improve the performance.}
AMOS~\cite{zheng2022amos} has optimized for TensorCore computation, covering FP16 and INT8 types, but it is specific to NVIDIA GPUs. In comparison, \oursys{} is the first compiler to optimize for general low-precision computations that support general custom data types on different GPUs.
Deep learning libraries or frameworks like ONNXRuntime~\cite{onnxruntime} and TensorRT~\cite{tensorrt} support some low-bit operators for inference scenarios, but their coverage is still limited due to the significant effort required to implement those combinatorial cases.
Some recent compilers like Triton~\cite{tillet2019triton} and TensorIR~\cite{feng2023tensorir} allow users to directly write the computation pipeline of a DNN operator, providing flexibility in specifying scheduling in each stage. However, these compilers mostly focus on computation scheduling and have little support in data scheduling for custom data types, which is the primary focus of \oursys{}.

\para{Model-specific low-precision optimization.}
Given the lacking efficient support of low-precision in existing compilers and frameworks, many works have conducted workload-specific low-precision optimizations. For example, some quantization and model training on low-precision types are optimized for Large Language Models (LLMs)~\cite{touvron2023llama, workshop2022bloom, frantar2022gptq, lin2023awq, rouhani2023microscaling, wang2023bitnet, ma2024era, vllm}. Previous work like ~\cite{he2016deep, huang2019efficient, ma2018shufflenet, shen2023efficient, gulati2020conformer} optimizes other models like ShuffleNet, Conformer, etc., into FP8 or FP16 precision.
In comparison, \oursys{} provides a mechanism to allow one to more easily implement custom data types and optimization policies. Thus, these optimization approaches are complementary to \oursys{}, as they can be implemented or automatically optimized in \oursys{}.

